Adapting to Evolving Adversaries with Regularized Continual Robust Training

Robust training methods typically defend against specific attack types, such as Lp attacks with fixed budgets, and rarely account for the fact that defenders may encounter new attacks over time. A natural solution is to adapt the defended model to new adversaries as they arise via fine-tuning, a method which we call continual robust training (CRT). However, when implemented naively, fine-tuning on new attacks degrades robustness on previous attacks. This raises the question: how can we improve the initial training and fine-tuning of the model to simultaneously achieve robustness against previous and new attacks? We present theoretical results which show that the gap in a model's robustness against different attacks is bounded by how far each attack perturbs a sample in the model's logit space, suggesting that regularizing with respect to this logit space distance can help maintain robustness against previous attacks. Extensive experiments on 3 datasets (CIFAR-10, CIFAR-100, and ImageNette) and over 100 attack combinations demonstrate that the proposed regularization improves robust accuracy with little overhead in training time. Our findings and open-source code lay the groundwork for the deployment of models robust to evolving attacks.

==> sections/2intro.tex <==
Research on designing attacks against image classification has led to a wide variety of attack types\citep{madry2017towards, XiaoZ0HLS18, LaidlawF19, laidlaw2020perceptual, wasserstein_attacks, wu2020stronger, brown2017adversarial}, such as $\ell_p$-bounded attacks \citep{madry2017towards}, spatial transformation based attacks \citep{XiaoZ0HLS18}, and color shift based attacks \citep{LaidlawF19}.  However, the scope of research on defending against multiple attacks simultaneously is limited in comparison. Existing work on defending against adversarial examples has focused primarily on achieving robustness against a single attack type (primarily $\ell_p$ bounded attacks) \citep{madry2017towards, zhang2019theoretically, croce2020robustbench, gowal2020uncovering, cohen2019certified,  gowal2021improving, sehwag2021robust}.  While a few works have looked at achieving robustness against multiple attacks \citep{MainiWK20, TB19, madaan2020learning, Croce020,croce2022adversarial}, a property we refer to as \emph{multi-robustness} for short, these works all assume that every attack we would like to be robust against is known \textit{a priori} by the defender.  This is unrealistic as it is difficult to model the space of perturbations we would like to be robust to, and over time, new perturbation types may be introduced.  Thus, it is important to consider a temporal dimension to the problem of multi-robustness; specifically, new attacks are introduced \textit{sequentially} and the defender can continuously update the deployed model to be robust against the new attack, while maintaining robustness on the previous attacks.  This dynamic setting of robustness is known as \textit{continual adaptive robustness} (CAR) \citep{dai2024position}.

\textbf{How can continual adaptive robustness be obtained? (\cref{sec: setup})} In CAR, it is important that models can be adapted quickly to new attacks when they are introduced.  While this setting was introduced by \citet{dai2024position}, to the best of our knowledge, no prior works have analyzed and proposed defenses in this setting.  We propose \textit{continual robust training} (CRT) as a natural solution for CAR.  CRT (Figure \ref{fig:overview}) consists of two main parts: (1) initial adversarial training, where we perform adversarial training to obtain robustness against the set of attacks known before deployment, and (2) iterative robust fine-tuning where each time a new attack is introduced post-deployment, we fine-tune the model to gain robustness against the new attack.

%Robustness to adversarial examples has emerged as one of the key requirements for the safe deployment of machine learning (ML) models. Most work on creating robust models has focused on adversarial examples generated via a single attack. Recently, there has been a push to make ML models robust to adversarial examples generated by multiple attacks \citep{MainiWK20, TB19, madaan2020learning, Croce020,croce2022adversarial}, which we refer to as \emph{multi-robustness} for short. Multi-robustness is critical for the practical deployment of robust models since practitioners will be unwilling to deploy an expensively trained model only for it to be vulnerable to the next attack that emerges. \christian{Minor point but I think plenty of practitioners are willing to deploy non-robust models.}

%\textbf{Paragraph 1}: Why should we care about multi-robustness - this is the only way robustness can be made practical. It is also intellectually challenging as it is harder than achieving singly robust models and can inform their design. prior work has however focused on the setting where all the attacks to be defended against are known simultaneoulsy

\begin{figure*}[!t]
	\centering
	\includegraphics[width=\textwidth]{figures/overview_figure_2.pdf}
	\caption{An overview of the problem of adapting to new adversaries (Continual Adaptive Robustness) and our solution framework (Regularized Continual Robust Training).  In this problem, the defender learns about the existence of new attacks sequentially, and at time $t$ aims to achieve robustness against all attacks seen at times $\le t$.  The model is deployed at time $0$ to be robust against an initial set of attacks, new attacks are introduced at times $t_1$, $t_2$, and $t_3$. We propose to performing initial robust training when the first attack (or set of attacks) is available and then use fine-tuning to adapt the model against future attacks within time $\Delta t$.}
	\label{fig:overview}
	\vspace{-20pt}
\end{figure*}

%\arjun{Paragraph below needs a rewrite. Start with multi-robustness being important, and then its relation to the problem of CAR and why we should care about it. Then, propose CRT as a natural solution. But, then ask, how is it best done? That's where our theory and RCRT comes in.}

%Not only does multi-robustness introduce extra computational considerations, it is often unclear whether joint robustness is even possible for attacks with very different constraint sets. Most prior work has focused on training models that are jointly robust against different $\ell_p$ adversaries \citep{MainiWK20, TB19, madaan2020learning}. The critical assumption here is that all the attacks that need to be defended against are known \emph{a priori}. In this paper, we consider the scenario where models are trained to be multi-robust one attack at a time, a paradigm known as Continual Adaptive Robustness \citep{dai2024position}. This is of interest for two reasons: i) new attacks are likely be revealed over time requiring model trainers to have a training strategy that accounts for them; ii) continual training improves efficiency by obviating the need to train from scratch with all attacks for each new attack, and can leverage the benefits of residual robustness, if any. Thus, the key question we ask in this paper is:

%\begin{center}
%\emph{How can a model trainer effectively and efficiently adapt to new attacks?}
%\end{center}

%\textbf{Paragraph 2}: Perhaps a more practical scenario is where different attacks reveal themselves over time. even if you know all attacks, you can benefit from residual robustness and reduce overall training time, and also not hit capacity by trying to train in too many attacks at the same time. Given this, we consider the paradigm of CAR, where the defender trains a model to be robust one attack at a time. The key question we ask is: how can a defender efficiently and effectively adapt to new attacks?

\noindent \textbf{Theoretical improvements via regularization (\cref{subsec: theory}):} A natural question to ask is: what changes to the training procedure can we make to best perform CRT?  The key challenges here are to obtain robust representations before each new attack is introduced that provide as much robustness to unseen attacks as possible, and to fine-tune with minimal degradation in robustness against previous attacks. Our theoretical analysis shows that the difference in robust losses with respect to a pair of attacks is upper bounded by a function of the \textit{adversarial sensitivity} of a model's representation function: the maximal $\ell_2$ distance between the representations of a data point and a perturbed version of that data point, given the two adversarial constraints.
% \sophie{unclear what adversarial sensitivity means, might help to mention L2 to make the connection to next paragraph more clear} 
As a corollary, we show the difference between the robust loss over the union of two attacks and the benign loss has the same upper bound. These results motivate regularizing robust representations to avoid loss degradation against previous attacks and to have acceptable performance on benign data.

\textbf{Regularization Methods (\cref{subsec: methods}):} Our theoretical results motivate the use of regularization in CRT, and thus, we propose Regularized CRT (RCRT) using \emph{adversarial $\ell_2$ regularization} during both robust pre-training and fine-tuning. This regularization term, motivated by our theoretical results, promotes closeness in terms of Euclidean distance between adversarial and benign representations. We also consider two potential variants to improve efficiency and robustness: i) \emph{Random Noise Regularization:} the representations used are generated using \emph{random noise} instead of worst-case adversarial perturbations; ii) \emph{Variation Regularization \citep{dai2022formulating}:} the Euclidean distance between representations resulting from different instantiations of the adversarial perturbation is minimized.

\noindent \textbf{Empirical Findings (\cref{sec: results}):} We conduct experiments on hundreds of attack combinations on 3 vision datasets to rigorously determine the multi-robustness of models trained using RCRT.  Interestingly, we observe that when used in initial training, all variants of regularization generally improve robustness on new attacks.  For example, using regularization based on uniform noise, we can improve robust accuracy on a spatial attack (StAdv \citep{XiaoZ0HLS18}) from 0.79\% to 26.22\% while training only with $\ell_2$ attacks on CIFAR-10.  We further observe that variants of regularization using adversarial perturbations (adversarial $\ell_2$ and variation regularization) generally improve robustness when used during fine-tuning.  For example, when fine-tuning a model initially robust to $\ell_2$ attacks, using adversarial $\ell_2$ regularization can improve robustness on the snow attack~\citep{kaufmann2019testing} by 7.85\% on ImageNette \citep{imagenette} (from 27.64\% to 35.49\%).%We compare these models to those trained using 3 baselines for continual robust training and 3 for simultaneous multi-robust training from prior work. While no single method dominates in all settings, we find that RCRT provides a good balance between performance and efficiency compared to existing methods for CRT. In addition, we find that CRT methods in general approach or even surpass simultaneous multi-robust training, while being much more efficient. \arjun{Maybe add a couple of illustrative numbers here Sophie?}

\noindent \textbf{Looking ahead (\cref{sec: discussion}):} We show how CAR can be effectively achieved using iterative fine-tuning and regularization techniques. However, future work is necessary to better understand how interactions between sets of adversarial constraints impact the joint learnability of different attacks. We hope that our RCRT method will help practitioners ensure that their models remain robust against changing real-world threats, and may be adapted to ensure other desirable properties, such as compliance with changing standards for fairness or privacy. 
% \sophie{privacy and fairness definitions don't change over time as it does with adversarial examples}


%\textbf{Paragraph 3:} The simple answer to this question is to just pre-train with a specific attack and then fine-tune . However, the robust loss on different attacks for the same classifier, even if jointly trained on both attacks, can be quite different. To control how large this term is, we first prove that the difference in the robust loss for different attacks is bounded by the distance between of the learned robust features. 

%\arjun{The direct way to use the theory is to just consider the classifier trained jointly on both type of adversaries, and then the motivation for regularization is clear. But what would be nicer is to say that if you regularize in pre-training, then you reduce the difference in loss for any subsequent classifier}

%\arjun{Why do continual over joint in practice should be the only argument we make. We should not explicitly say that we are trying to beat joint, just get in the ballpark.}



%In this work, we study a new direction in adversarial robustness called \probname ~(\probabbrv) \sophie{add citation once position paper is up on arxiv}.  In \probabbrv, attacks are introduced in a sequential manner after the defender's model is deployed.  The goal of the defender is to quickly adapt the deployed model to be robust against the new attack while retaining robustness against all previous attacks in the sequence.

%To address this problem, we propose using an initial training and fine-tuning framework which involves first performing adversarial training with the initial attack and then fine-tuning for a few epochs on examples using new attacks once they are introduced (Figure \ref{fig:overview}).  We demonstrate that regularization is crucial for this problem \sophie{add more details here}

% Old text
%While existing machine learning (ML) models can achieve high accuracy, they are vulnerable to imperceptible perturbations in the input space called adversarial examples \citep{szegedy2013intriguing}.  These perturbations can be exploited by an attacker in order to cause misclassification, which may be harmful in safety critical areas.

%Prior works in adversarial robustness consider designing defenses for achieving robustness against a single attack type.  For example, many works propose defenses for achieving robustness against an attacker using a bounded $\ell_\infty$ or $\ell_2$ attack \citep{cohen2019certified, madry2017towards, zhang2019theoretically}.  However, these attacks can only capture a small portion of the space of possible perturbations; many works in attack literature have proposed other forms of attacks that are not captured by the $\ell_p$ threat model \citep{XiaoZ0HLS18, LaidlawF19, laidlaw2020perceptual, kaufmann2019testing}.  This motivates the design of a defense that can be efficiently adapted over time to new attacks.

==> sections/checklist.tex <==
\clearpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
%limit. 

%Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
%\begin{itemize}
%    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
%\end{itemize}

%{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

%The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

%IMPORTANT, please:
%\begin{itemize}
%    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
%\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Claims are substantiated by theoretical (Section~\ref{subsec: theory}) or empirical (Section~\ref{sec: results}) results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section \ref{sec: discussion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our theoretical assumptions for Theorem~\ref{thm:robustness} and Corollary~\ref{thm:corollary} are provided in Section~\ref{subsec: theory}, and full proofs of these two results are provided in Appendix~\ref{sec:proof}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Full details of our training method and regularization terms are provided in Sections~\ref{sec:regularization},~\ref{sec:exp_setup} and Appendix~\ref{app:exp_setup}. We make use of established model architectures (ResNet18 and WideResNet28-10) and publicly-available datasets (CIFAR-10, CIFAR-100, and ImageNette).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We are attaching code to reproduce our experiments in our initial submission, and will make our code available in a public repository by the time of publication. We use only publicly-available datasets in our experiments (CIFAR-10, CIFAR-100, and ImageNette).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Full details of our training method and regularization terms are provided in Sections~\ref{sec:regularization},~\ref{sec:exp_setup} and Appendix~\ref{app:exp_setup}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Due the the scale of our experimentation, we did not have the computational resources to to report error bars for all experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Training time is reported as a relevant metric for the models we train and is a key contribution of our training method.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work conforms with the NeurIPS Code of Ethics. We do not perform human subjects research and only use public datasets. Any potential downstream harms of our work are discussed in the broader impact section (\cref{sec: discussion}).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section \ref{sec: discussion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks.%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The model architectures and datasets we use are properly cited and attributed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not release any new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing or research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing or research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}
